REFINE: Reachability-based Trajectory Design using Robust Feedback Linearization and Zonotopes

Performing real-time receding horizon motion planning for autonomous vehicles while providing safety guarantees remains difficult. This is because existing methods to accurately predict ego vehicle behavior under a chosen controller use online numerical integration that requires a fine time discretization and thereby adversely affects real-time performance. To address this limitation, several recent papers have proposed to apply offline reachability analysis to conservatively predict the behavior of the ego vehicle. This reachable set can be constructed by utilizing a simplified model whose behavior is assumed a priori to conservatively bound the dynamics of a full-order model. However, guaranteeing that one satisfies this assumption is challenging. This paper proposes a framework named REFINE to overcome the limitations of these existing approaches. REFINE utilizes a parameterized robust controller that partially linearizes the vehicle dynamics even in the presence of modeling error. Zonotope-based reachability analysis is then performed on the closed-loop, full-order vehicle dynamics to compute the corresponding control-parameterized, over-approximate Forward Reachable Sets (FRS). Because reachability analysis is applied to the full-order model, the potential conservativeness introduced by using a simplified model is avoided. The pre-computed, control-parameterized FRS is then used online in an optimization framework to ensure safety. The proposed method is compared to several state of the art methods during a simulation-based evaluation on a full-size vehicle model and is evaluated on a 1/10th race car robot in real hardware testing. In contrast to existing methods, REFINE is shown to enable the vehicle to safely navigate itself through complex environments.

==> sections/AWD.tex <==
\section{Generalization to All-Wheel-Drive}
\label{sec: AWD}
Desired controller and planning strategy introduced so far can be generalized for All-Wheel-Drive (AWD) vehicles.
Compared to FWD vehicles, AWD vehicles share the same dynamics as in Section \ref{sec: dynamics} except only lateral rear tire force is estimated and all the other three tire forces are controlled by proper tire speed and steering angle.

In particular, any computation related to lateral tire forces remains the same, but both front and rear tires contribute nonzero longitudinal tire forces satisfying linear equalities $l_\text{f}F_\text{xf}(t) = l_\text{r}F_\text{xr}(t)$ and 
\begin{equation}
    F_\text{xf}(t) + F_\text{xr}(t) = m\duexp(t,p;d) -mv(t)r(t) + m\varphi_u(t,p;d).
\end{equation}
Furthermore the validation of Assumption \ref{ass: small slip} for AWD vehicles needs to consider both slip ratios via
\begin{equation}
    \lambda_\text{f}(t) = \lambda_\text{r}(t) = \frac{\duexp(t,p;d) -v(t)r(t) + \varphi_u(t,p;d)}{g \bar\mu}.
\end{equation}


==> sections/RTDandFRS_COPY.tex <==
\section{Reachability-based Trajectory Design and Reachability Analysis}
\label{sec: rtd}

To address safety concerns during vehicle motion planning, we extend the Reachability-based Trajectory Design (RTD) method \cite{kousik2020bridging}, which consists of offline reachability analysis and online planning.
This section begins by describing RTD at a high-level and describes how we extend it in \methodname{}.
Then it describes the offline reachability analysis on the ego vehicle as a state-augmented hybrid system using zonotopes and illustrates how the ego vehicle's footprint can be accounted for during reachability analysis.

\subsection{Reachability-based Trajectory Design and \methodname{}}
During offline computation of RTD, the FRS of the vehicle dynamics with parameterized control inputs is conservatively approximated.
The FRS includes all possible behaviors of the ego vehicle over a finite time horizon and is mathematically defined in Section \ref{subsec: FRS computation}.
During online planning, RTD performs control synthesis by solving optimization problems in a receding horizon fashion, where the optimization searches for the optimal trajectory parameter for navigating the ego vehicle to some waypoint while behaving in a not-at-fault manner. 

Note in \methodname{} we similarly pre-compute and apply reachability analysis as in RTD; however, in contrast to RTD, which performs reachability analysis on a simplified vehicle model using SOS programming, \methodname{} performs reachability analysis on a realistic vehicle model. 
To ensure that this reachability analysis can generate tight, overapproximative representations of the FRS of the vehicle dynamics, \methodname{} relies on the controller design described in Section \ref{sec: controller}.
Because this controller partially linearizes the dynamics, \methodname{} relies on a zonotope-based reachable set representation which works well to describe the FRS of nearly linear dynamical systems. 
% Such a waypoint is usually generated by a high level trajectory planner, such as a Rapidly-Exploring Random Tree \cite{lavalle2001randomized}. 

As in Assumption \ref{ass: sense horizon}, each planning iteration in \methodname{} is allotted $\tplan>0$ time to generate a plan.
If a particular planning iteration begins it computation at time $t_0$, its goal is to find a control policy by solving an online optimization within $\tplan$ seconds so that the control policy can be applied during the time interval $[t_0+\tplan, t_0+\tplan+ \tf]$.
\Review{As a result of Lemma \ref{lem:braking}}{Because any parametrized trajectory in Definition \ref{def:traj_param} breaks the ego vehicle to a stop in the end}, it is natural to partition the time interval $[t_0+\tplan, t_0+\tplan+ \tf]$ into $[t_0+\tplan,t_0+\tplan+\tnb)$ during which a non-braking maneuver is \Review{applied}{tracked} and $[t_0+\tplan+\tnb,t_0+\tplan+\tf]$ during which a braking maneuver is activated\jinsun{$\tnb$ has nothing to do with Lemma \ref{lem:braking}}.
\Review{}{Note the reference trajectory of the vehicle speed during braking can gradually decrease the speed first, then become 0.
Thus $\tnb$ is not necessarily equal to $\tstop$.}
\Review{Note}{As a result of Lemma \ref{lem:braking},} by setting $\tf$ equal to \Review{$\tnb + \tb$}{ $\tb$} one can guarantee that the ego vehicle comes to a complete stop by $\tf$.
To simplify the notation, from now on we reset time to $0$ whenever a feasible control policy is about to be applied. \jinsun{should we move the last sentence to the end of next paragraph?}

% \begin{figure}[h]
%     \centering
%     \includegraphics[trim={0cm, 1.8cm, 3.5cm, 3.2cm},clip,width=\columnwidth]{figures/timeline.pdf}
%     \caption{Explanation of online planning. Non-braking and barking maneuvers are plotted in red and blue. 
%     Duration of maneuvers that are being planned at current planning iteration are marked as solid line segments. 
%     Planned maneuvers are marked as dashed line segments if they are applied to ego vehicle. 
%     \jinsun{may need to change color later. Also I'm hesitating of keeping this plot, since it is not necessary, but I figure this plot can be helpful when I explain RTD to other people. So help me decide...}}
%     \label{fig:timeline}
% \end{figure}

Suppose the planning iteration at time $\tz$ is feasible (i.e., not-at-fault), then the feasible control policy starts being applied at $\tz+\tplan$.
% Meanwhile another planning iteration will start at time $t_0+\tplan+\tnb-\tplan = t_0+\tnb$, and the same planning procedure repeats.
However if the planning iteration starting at time $\tz$ is infeasible, then the braking maneuver, whose safe behavior was verified in the previous planning iteration, can be applied starting at $\tz+\tnb$ to bring the ego vehicle to a stop in a not-at-fault manner.
Therefore to ensure real-time performance, $\tplan\leq\tnb$ \Review{}{needs to hold}.

% \Ram{may be move the remainder of this subsection into the online optimization section.}
% Algorithm \ref{alg: RTD} summarizes the .... 
% Notice that lines from 2 to 8 in Algorithm \ref{alg: RTD} are just to ensure that the first planning iteration has a feasible plan so that a safe braking maneuver is available if the following planning iteration fails.

% \begin{algorithm}[t]
%     \caption{RTD Planning}
%     \label{alg: RTD}
%     \begin{algorithmic}[1]
%         \REQUIRE $\tplan$, $\tnb$, FRS \texttt{//FRS is conservatively approximated in Sec. \ref{subsec: FRS computation}}
%         \STATE $t_0\gets$ current time
%         \STATE \textbf{sense} obstacles
%         \STATE \textbf{compute} $(p,d)\gets$ OnlineOptimization(FRS) \\ \texttt{//see Alg. \ref{alg: OnlineOpt} in Sec. \ref{sec: bin idea}}
%         \IF{no feasible $(p,d)$}
%             \RETURN \texttt{//no feasible plan, so stop}
%         \ENDIF
%         \STATE \textbf{execute} non-braking maneuver parameterized by $(p,d)$ at time $t_0+\tplan$
%         \STATE $t_0\gets t_0+\tnb$, $(p_\text{pre}, d_\text{pre})\gets(p,d)$
%         \WHILE{true}
%             \STATE \textbf{sense} obstacles
%             \STATE \textbf{compute} $(p,d)\gets$ OnlineOptimization(FRS) \\ \texttt{// repeat planning} 
%             \IF{no feasible $(p,d)$}
%                 \STATE \textbf{execute} braking maneuver parameterized by $(p_\text{pre}, d_\text{pre})$ at time $t_0+\tplan$ \\ \texttt{//brake the ego vehicle}
%                 \RETURN  \texttt{//stop planning}
%             \ENDIF
%             \STATE \textbf{execute} non-braking maneuver parameterized by $(p,d)$ at time $t_0+\tplan$
%             \STATE $t_0\gets t_0+\tnb$, $(p_\text{pre}, d_\text{pre})\gets(p,d)$
%         \ENDWHILE
%     \end{algorithmic}
% \end{algorithm}

% To simplify the notation, from now on we reset time to 0 whenever a feasible control policy is about to be applied, i.e. $t_0+\tplan \equiv 0$.


% \subsection{Augmented States and Hybrid System}
% \label{subsec:hybrid_desc}

% Our goal is to compute the predicted ego vehicle behavior starting from some initial condition $z_0\in\Z_0\subset\R^6$, i.e. $\zhi(0)=z_0$ or $\zlo(0)=\pi_{1:4}(z_0)$ depending on the value of the 4th dimension in $z_0$.
% To simplify the reachability computation in the next subsection, we augment the initial condition $z_0$ and control parameter $p$ into the vehicle state vector as $\zaug(t) = [x(t),y(t),h(t),u(t),v(t),r(t),z_0^\top, p^\top]^\top\in\R^6\times\Z_0\times\P\subset\R^{14}$ in which the last 8 dimensions are static with respect to time. 
% Then dynamics of the augmented vehicle state during high-speed and low-speed scenarios can be written as
% \begin{equation}
% \label{eq: dyn tilde_z}
%     \dzaug(t) = \begin{dcases}
%         \begin{bmatrix}
%             \fhi(t,\zhi(t),p;d) \\ 0_{8\times1}
%         \end{bmatrix} , \text{ if } u(t) > \uc, \\ \\
%         \begin{bmatrix}
%             \flo(t,\zlo(t),p;d) \\ 0_{10\times1}
%         \end{bmatrix} , \text{ if } u(t) \leq \uc.
%     \end{dcases}
% \end{equation}
% Notice when $u(t)\leq \uc$, assigning fake zero dynamics to $v$ and $r$ in \eqref{eq: dyn tilde_z} does not affect the evolution of the vehicle's dynamics because the lateral speed and yaw rate are directly computed via longitudinal speed as in \eqref{eq: r lo} and \eqref{eq: v lo}.

% Because the vehicle's dynamics vary based on $u(t)$, it is natural to model the ego vehicle as a hybrid system $HS(d)$ for each $d\in\{1,2,3\}$. 
% Each hybrid system has $\zaug(t)$ as its state and consists of a high-speed mode and a low-speed mode with dynamics in \eqref{eq: dyn tilde_z}.
% Instantaneous transition among modes of $HS(d)$ are described using the notation of a \emph{guard} and \emph{reset map}.
% The guard triggers a transition and is defined as $\{\zaug(t)\in\R^6\times\Z_0\times\P\mid u(t) =\uc\}$. 
% Once a transition happens, the reset map maintains the last 8 dimensions of $\zaug(t)$, but resets the first 6 dimensions of $\zaug(t)$ via \eqref{eq: reset h2l} if $u(t)$ approaches $\uc$ from above and via \eqref{eq: reset l2h} if $u(t)$ approaches $\uc$ from below. 






\subsection{Offline FRS Computation}
\label{subsec: FRS computation}

The \emph{Forward Reachable Set (FRS)} of the ego vehicle is defined as
\begin{equation}
 \label{eq: FRS def}
\begin{split}
    \FRS([0,&\tf])=\Bigg\{(x,y)\in \W\mid \exists t\in[0,\tf], p\in\P,  \\
    & z_0\in\Z_0 \text{ s.t. }\begin{bmatrix} x\\ y \end{bmatrix} = \pi_{xy}(\zaug(t)), \zaug \text{ is a}   \\
    & \text{ solution of } HS \text{ with } \zaug(0)= \begin{bmatrix} z_0 \\  z_0 \\ p \end{bmatrix} \Bigg\},
\end{split}
 \end{equation}
where $\pi_{xy}:\R^{12+n_p}\rightarrow \R^2$ is the projection operator that outputs the first two coordinates from its argument.
$\FRS([0,\tf])$ collects all possible behavior of the ego vehicle while following the dynamics of $HS$ in the $xy$-plane over time interval $[0,\tf]$ for all possible $p\in\P$ and initial condition $z_0\in\Z_0$.
Computing $\FRS([0,\tf])$ precisely is numerically challenging because the ego vehicle is modeled as a hybrid system with nonlinear dynamics, thus we aim for finding an outer-approximation of $\FRS([0,\tf])$ instead.

To outer-approximate $\FRS([0,\tf])$, we start by assuming $\Z_0$ as a 6-dimensional box $\text{int}(\underline{z_0}, \overline{z_0}) = \zonocg{c_{0}}{G_0}$ where $c_0 = \frac{1}{2}(\underline{z_0}+\overline{z_0})$ and $G_0 = \frac{1}{2}\diag(\overline{z_0}-\underline{z_0})$.
Recall that because $\P$ is a compact n-dimensional box, it can also be represented as a zonotope as $\zonocg{c_p}{G_p}$ where $c_p = \frac{1}{2}(\underline p+\overline p)$ and $G_p = \frac{1}{2}\diag(\overline p - \underline p)$. 
Then the initial conditions for $\zaug(0)$ can be represented as a zonotope $\Zaug_0=\zonocg{c_{\zaug}}{G_{\zaug}} \subset \Z_0\times\Z_0\times\P$ where 
\begin{equation}
    c_{\zaug} = \begin{bmatrix}
    c_0\\ c_0\\ c_p
    \end{bmatrix}, ~ G_{\zaug} = \begin{bmatrix}
    G_0 & 0_{6\times n_p}\\ G_0 & 0_{6\times n_p} \\ 0_{n_p \times6} & G_p
    \end{bmatrix}.
\end{equation}
% \simon{this initially confused me a lot (but eventually it was clear. Do we really need what $\tilde{\Z}_0$ is?}\jinsun{I think we need this to initialize the computation.}
Observe that by construction each row of $G_{\zaug}$ only has 1 nonzero element. 
% Then dynamics of the augmented vehicle state during high-speed and low-speed scenarios is
% \begin{equation}
% \label{eq: dyn tilde_z}
%     \frac{d}{dt}\tilde z(t) = \begin{cases}
%         \begin{bmatrix}
%             \xi_\text{hi}(t,z_\text{hi}(t),p,d) \\ 0_{8\times1}
%         \end{bmatrix} , \text{ if } u(t) > u_c, \\ \\
%         \begin{bmatrix}
%             \xi_\text{lo}(t,z_\text{lo}(t),p,d) \\ 0_{10\times1}
%         \end{bmatrix} , \text{ if } u(t) \leq u_c.
%     \end{cases}
% \end{equation}
% Notice when $u(t)\leq u_c$, \eqref{eq: dyn tilde_z} assigns \simon{maybe delete fake?}\jinsun{I use `fake' because I want to emphasize that $v$ and $r$ don't really have zero dynamics, but this fake zero dynamics doesn't affect the way we evaluate $u$ and $v$ in low speed model.} fake zero dynamics to $v(t)$ and $r(t)$ which do not affect the evolution of vehicle dynamics.

Next we pick a time step $\Delta_t\in\R_+$ such that $\tau/\Delta_t\in\N$, and partition the time interval $[0,\tf]$ into $\tf/\Delta_t$ \emph{time segments} as $T_j=[(j-1)\Delta_t, j\Delta_t]$ for each $j\in \J=\{1,2,\cdots,\tf/\Delta_t\}$.
\Review{Finally, we use an open-source toolbox Cora \cite{althoff2015introduction}, which takes the $HS$ model of the system and the set of initial conditions $\Zaug_0$, and computes $\RR_j$ for each $j \in \J$ where $\FRS(T_j) \subset \RR_j$}{} \Ram{need to write this as a theorem and cite a specific theorem from Althoff's papers} \jinsun{addressed} 
\Review{Note that this can be done offline and then used online. 
In fact, one can prove that $\FRS([0,\tf])\subseteq\cup_{j\in \J}\pi_{xy}\left(\RR_j\right)$.}{}
\Review{}{Finally we use an open-source toolbox CORA \cite{althoff2015introduction}, which takes $HS$ and the set of initial conditions $\Zaug_0$, to over-approximate the FRS in \eqref{eq: FRS def} by a collection of zonotopes $\{\RR_j\}_{j\in\J}$ over all time intervals where $\RR_j\in\R^{12}\times\P$.
As a direct application of Theorem 3.3, Proposition 3.7 and the derivation in Section 3.5.3 in \cite{althoff2010reachability}, one can conclude the following theorem:}
\begin{thm}
\label{thm: FRS over-approximation}
\Review{}{The zonotope $\RR_j\subset\R^{12}\times\P$ computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$ ensures $\zaug(t) \in\RR_j$ for all $j\in\J$ and $t\in T_j$, therefore}
\begin{equation}
    \Review{}{\FRS([0,\tf]) \subset \bigcup_{j\in\J}\pi_{xy}(\RR_j).}
\end{equation}
\end{thm}





% Computation of such zonotope $\RR_j(d)$ is detailed in \cite[Section 3.5]{althoff2010reachability} \Ram{please cite a particular theorem that proves that its an outerapproximation for hybrid systems}, and for simplicity denote $\RR_\J(d)$ the collection of $\RR_j(d)$ for all $j\in\J$.
% Relation \eqref{eq: R_int} together with definition of FRS directly infer that
% \begin{equation}
%     \mathcal Z_{xy}(d)\subseteq\cup_{j\in \J}\pi_{xy}\left(\RR_j(d)\right).
% \end{equation}

% Let $\tilde\Z_0^d=\tilde\Z_0$ for all $d\in\{1,2,3\}$, then FRS computation can be considered in the following 3 scenarios using augmented vehicle state space.

% \begin{enumerate}
%     \item \textit{No Transition Occurrence:}
%     For any $j\in\{1,\cdots,T/\Delta_t\}$, suppose $\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1}^d\subset\R^{14}$ where $\tilde\Z_{j-1}^d$ is some given zonotope.
%     Then treating $\tilde\Z_{j-1}^d$ as the initial condition of $T_j$ and ignoring any transition between the high-speed and low-speed models, one can use an open-source toolbox Cora \cite{althoff2015introduction} with initial condition $\tilde\Z_{j-1}^d$ of $T_{j-1}$, time step $\Delta_t$ and augmented dynamics \eqref{eq: dyn tilde_z} to compute two zonotopes $\tilde\Z_{j}^d,\tilde\RR_j^d\subset\R^{14}$ such that
%     \begin{align}
%         \{\tilde z(j\Delta_t)\mid \tilde z((j-1)&\Delta_t)\in\tilde\Z_{j-1}^d,\\
%         &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}}\}\subset\tilde\Z_{j}^d\nonumber
%     \end{align}
%     and 
%     \begin{align}
%     \{\tilde z(t)\in\R^{14}\mid &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1}^d, \label{eq: FRS no trans}\\
%         &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}},~ t\in T_j\}\subset \tilde\RR_j^d.\nonumber
%     \end{align}
%     Details of zonotope computation and these two relations are described in \cite[Section 3.4]{althoff2010reachability}.
%     It is straightforward to see $\tilde\Z_{j-1}^d\subset\tilde\RR_j^d$ and $\tilde\Z_{j}^d\subset\tilde\RR_j^d$.
    
%     Denote $\pi_u:\R^{14}\rightarrow \R$ the projection operator as $\pi_u(\tilde z(t))\mapsto u(t)$.
%     If $u_c\notin\pi_u(\tilde\RR_j^d)$, then indeed no transition between the high-speed and low-speed models happens during $T_j$.
%     Thus the same computation and check of membership can be repeated iteratively among successive time segments until $u_c\in\pi_u(\tilde\RR_{j'}^d)$ for some integer $j'>j$.
%     For simplicity call $\tilde\Z_{j}$ the \emph{FRS of $\tilde z$ at time $j\Delta_t$}, and call $\tilde\RR_{j}^d$ the \emph{FRS of $\tilde z$ over $T_j$}.
    
%     \item \textit{High-speed to Low-speed Transition:}
%     A transition from high-speed model to low-speed model may happen during $T_j$ if $u_c\in\tilde\Z_0^d$ and $j=1$\simon{why j = 1 is useful}\jinsun{because you may start with a speed around $u_c$}, or if $u_c\in\pi_u(\tilde\RR_j^d)$ and $(0,u_c]\cap\pi_u(\tilde\Z_{j-1}^d)=\emptyset$ with $j>1$ where $\tilde\Z_{j-1}^d$ and $\tilde\RR_j^d$ are either given or computed zonotopes via the high-speed portion of \eqref{eq: dyn tilde_z}.\simon{maybe we can do 36.1, 36.2 to not refer to high-speed and low-speed so many times} \jinsun{good idea. could you make the change?}
%     % Suppose $u_c\in\pi_u(\tilde\RR_j)$ but $(0,u_c]\cap\pi_u(\tilde\Z_{j-1})=\emptyset$, then a transition from high-speed model to low-speed model may happen during the $j$-th time segment.
%     Notice the occurrence of transition during $T_j$ cannot be confirmed since both $\tilde\Z_{j-1}^d$ and $\tilde\RR_j^d$ are outer-approximations of $\tilde z(t)$ at time $(j-1)\Delta_t$ and over $T_j$ respectively.
%     To locate the transition time $\ttrans^{\text{h2l},d}$ where the supscript `h2l' means `high-to-low', one can keep computing the FRS of $\tilde z$ with only the high-speed portion of \eqref{eq: dyn tilde_z} until $[u_c,+\infty)\cap\pi_u(\tilde\RR_{j'+1}^d)=\emptyset$ for some integer $j'>j$, therefore $\ttrans^{\text{h2l},d}\in T_j\cup T_{j+1}\cup\cdots\cup T_{j'}$.
%     If no such $j'$ exists, set $j'$ as \simon{maybe add: the last time instant}\jinsun{done} the last time instant $T/\Delta_t$.
%     One can then use Cora with initial condition $\tilde\Z_{j-1}^d$ of $T_{j-1}$,\simon{maybe add: a large}\jinsun{ok} a large time step $(j'-j+1)\Delta_t$ and the high-speed portion of augmented dynamics \eqref{eq: dyn tilde_z} to compute a zonotope $\tilde \RR_{(j,j')}^{\text{hi},d}$ such that 
%     \begin{align}
%         \{\tilde z&(t)\in\R^{14}\mid \frac{d}{dt}\tilde z(t)=[\xi_\text{hi}^\top(t,z_\text{hi}(t),p,d),0_{1\times 8}]^\top,\nonumber\\
%         &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1}^d,t\in T_j\cup\cdots\cup T_{j'}\}\subset \tilde \RR_{(j,j')}^{\text{hi},d}. \label{eq: h2l-hi}
%     \end{align}
%     Notice $(j'-j+1)\Delta_t$ is the duration of $T_j\cup\cdots\cup T_{j'}$, thus $\tilde z(\ttrans^{\text{h2l},d})\in\tilde \RR_{(j,j')}^{\text{hi},d}$.
    
%     Since augmented state $\tilde z$ should evolve \simon{maybe change to: with low-speed dynamics in 36}the low-speed portion of \eqref{eq: dyn tilde_z} after $\ttrans^{\text{h2l},d}$, we again use Cora with initial condition $\tilde\RR_{(j,j')}^{\text{hi},d}$, time step $\Delta_t$ and the low-speed portion of augmented dynamics \eqref{eq: dyn tilde_z} to iteratively compute zonotopes $\tilde\RR_j^{\text{lo},d},\tilde\RR_{j+1}^{\text{lo}d},\cdots,\tilde\RR_{j'}^{\text{lo},d}$ over time segments from $T_j$ to $T_{j'}$ such that $\tilde\RR_{(j,j')}^{\text{lo},d}\subset\tilde\RR_j^{\text{lo},d}\cup\cdots\cup\tilde\RR_{j'}^{\text{lo},d}$ where
%     \begin{align}
%         \tilde\RR_{(j,j')}^{\text{lo},d} = \{\tilde z(t)\mid &\tilde z((j-1)\Delta_t)\in\tilde\RR_{(j,j')}^{\text{hi},d},t\in\cup_{i=j}^{j'} T_i,\nonumber\\
%         &\frac{d}{dt}\tilde z(t)=[\xi_\text{lo}^\top(t,z_\text{lo}(t),p,d),0_{1\times 10}]^\top\}.
%     \end{align}
%     We point out that $\tilde \RR_{(j,j')}^{\text{hi},d}$ can be used to initiate the low-speed model because of \eqref{eq: reset h2l}, $\tilde z(\ttrans^{\text{h2l},d})\in\tilde \RR_{(j,j')}^{\text{hi},d}$ and the fact that the 5th and 6th dimensions of $d\tilde z(t)/dt$ with $u(0)\leq u_c$ as in \eqref{eq: dyn tilde_z} are fake zero dynamics. 
%     The following theorem gives the reachability analysis from time $(j-1)\Delta_t$ to $j'\Delta_t$.
%     \jinsun{Definitely need a explanation plot here}
%     \begin{lem}
%         \label{lem: h->l}
%         Let $\tilde\RR_{(j,j')}^{\text{h2l},d}:= \tilde\RR_{(j,j')}^{\text{hi},d}\cup \tilde\RR_j^{\text{lo},d}\cup\cdots\cup\tilde\RR_{j'}^{\text{lo},d}$\simon{why not have some symmetry here}\jinsun{you mean?}, then 
%         \begin{align}
%             \{\tilde z(t)\in\R^{14}\mid &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1}^d,\\
%         &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}},~ t\in\cup_{i=j}^{j'} T_i\}\subset \tilde\RR_{(j,j')}^{\text{h2l},d}.\nonumber
%         \end{align}
%     \end{lem}
%     % \begin{lem}
%     % \label{lem: h->l}
%     %     Suppose a high-speed to low-speed transition happens at time $\ttrans^\text{h2l}\in((j-1)\Delta_t, j'\Delta_t)$.
%     %     Then there exist zonotopes $\RR_{j,j'}^\text{hi}, \tilde\RR_j^\text{lo},\tilde\RR_{j+1}^\text{lo},\cdots,\tilde\RR_j^\text{lo}\subset\R^{14}$ such that
%     %     \begin{align}
%     %         \{\tilde z(t)\in\R^{14}\mid &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1},\\
%     %     &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}},~ t\in\cup_{i=j}^{j'} T_i\}\subset \tilde\RR_{j,j'}\nonumber
%     %     \end{align}
%     %     where 
%     %     $\tilde\RR_{j,j'}= \RR_{j,j'}^\text{hi}\cup \tilde\RR_j^\text{lo}\cup\cdots\cup\tilde\RR_{j'}^\text{lo}$.
        
%     %     % Define $\tilde\RR_{(j,j')}:= \RR_{j,j'}^\text{hi}\cup \tilde\RR_j^\text{lo}\cup\cdots\cup\tilde\RR_{j'}^\text{lo}$, then 
%     %     % \begin{align}
%     %     %     \{\tilde z(t)\in\R^{14}\mid &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1},\\
%     %     % &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}},~ t\in\cup_{i=j}^{j'} T_i\}\subset \tilde\RR_{(j,j')}.\nonumber
%     %     % \end{align}
%     % \end{lem}
    
%     \begin{proof}
%     % Construction of zonotopes $\RR_{j,j'}^\text{hi}, \tilde\RR_j^\text{lo},\tilde\RR_{j+1}^\text{lo},\cdots,\tilde\RR_j^\text{lo}$ has already been discussed.
%     The claim follows from \eqref{eq: h2l-hi}, $\tilde z(\ttrans^{\text{h2l},d})\in\tilde \RR_{(j,j')}^{\text{hi},d}$ and $\tilde\RR_{(j,j')}^{\text{lo},d}\subset\tilde\RR_j^{\text{lo},d}\cup\cdots\cup\tilde\RR_{j'}^{\text{lo},d}$.
%     \end{proof}
    
    
    
%     \item \textit{Low-speed to High-speed Transition:}
%     A transition from low-speed model to high-speed model may happen during $T_j$ if $u_c\in\tilde\Z_0^d$ and $j=1$, or if $u_c\in\pi_u(\tilde\RR_j^d)$ and $[u_c,+\infty)\cap\pi_u(\tilde\Z_{j-1}^d)=\emptyset$ with $j>1$ where $\tilde\Z_{j-1}^d$ and $\tilde\RR_j^d$ are either given or computed zonotopes via the low-speed portion of \eqref{eq: dyn tilde_z}.
%     % Suppose $u_c\in\pi_u(\tilde\RR_j)$ but $[u_c,\infty)\cap\pi_u(\tilde\Z_{j-1})=\emptyset$, then a transition from low-speed model to high-speed model may happen during the $j$-th time segment.
%     In this case reachability analysis is very similar as the computation in the case of \textit{High-speed to Low-speed Transition} except 
%     \begin{itemize}
%         \item we need to propagate $\tilde\Z_{j-1}^d$ with the low-speed portion of augmented dynamics \eqref{eq: dyn tilde_z} first, then its high-speed portion;
%         \item the post-transition dynamics needs to be initialized based on \eqref{eq: reset l2h}, not \eqref{eq: reset h2l}.
%     \end{itemize}
%     Such initialization of post-transition dynamics can be achieved in Cora by treating \eqref{eq: reset l2h} as a one-step discrete-time nonlinear system as in \cite[Section 9.5]{cora2018}.
%     Similar to Lemma \ref{lem: h->l}, the following lemma holds. 
    
%     \begin{lem}
%     \label{lem: l->h}
%         Suppose a low-speed to high-speed transition happens at time $\ttrans^{\text{l2h},d}\in((j-1)\Delta_t, j'\Delta_t)$ for some integer $j'\in(j,T/\Delta_t]$.
%         Then there exist zonotopes $\tilde\RR_{(j,j')}^{\text{lo},d}, \tilde\RR_j^{\text{hi},d},\tilde\RR_{j+1}^{\text{hi},d},\cdots,\tilde\RR_j^{\text{hi},d}\subset\R^{14}$ such that
%         \begin{align}
%             \{\tilde z(t)\in\R^{14}\mid &\tilde z((j-1)\Delta_t)\in\tilde\Z_{j-1}^d,\\
%         &\frac{d}{dt}\tilde z(t) \text{ as in \eqref{eq: dyn tilde_z}},~ t\in\cup_{i=j}^{j'} T_i\}\subset \tilde\RR_{(j,j')}^{\text{l2h},d}\nonumber
%         \end{align}
%         where 
%         $\tilde\RR_{(j,j')}^{\text{l2h},d}= \tilde\RR_{(j,j')}^{\text{lo},d}\cup \tilde\RR_j^{\text{hi},d}\cup\cdots\cup\tilde\RR_{j'}^{\text{hi},d}$.
%     \end{lem}
    

% \end{enumerate}

% \simon{do we need to distinguish l2h and h2l, can you just put all of them in R trans?}\jinsun{I think this is clearer than having R trans?}
% For any $d\in\{1,2,3\}$, let set $\J^d\subset\{1,2,\cdots,T/\Delta_t\}$ collect all possible indices of time segments during which no transition happens, set $\J^{\text{h2l},d}\subset \{1,2,\cdots,T/\Delta_t\}^2$ collect all possible index pairs of the form $j^\text{h2l} = (j_1^\text{h2l},j_2^\text{h2l})$ such that a high-speed to low-speed transition happens during  $((j_1^\text{h2l}-1)\Delta_t,j_2^\text{h2l}\Delta_t)$, and set $\J^{\text{l2h},d}\subset \{1,2,\cdots,T/\Delta_t\}^2$ collect all possible index pairs of the form $j^\text{l2h} = (j_1^\text{l2h},j_2^\text{l2h})$ such that a high-speed to low-speed transition happens during  $((j_1^\text{l2h}-1)\Delta_t,j_2^\text{l2h}\Delta_t)$.
% Denote $\pi_{xyp}:\R^{14}\rightarrow \R^4$ the projection operator as $\pi_{xyp}(\tilde z(t))\mapsto [x(t),y(t),p(t)^\top]^\top$, then the following theorem follows directly from \eqref{eq: FRS no trans}, Lemma \ref{lem: h->l} and Lemma \ref{lem: l->h}.
% \begin{thm}
%     \label{thm: FRS cover}
%     For any $d\in\{1,2,3\}$, $j\in\J^d$, $j^\text{h2l}=(j_1^\text{h2l},j_2^\text{h2l})\in\J^{\text{h2l},d}$ and $j^\text{l2h}=(j_1^\text{l2h},j_2^\text{l2h})\in\J^{\text{l2h},d}$, there exist zonotope $\tilde\RR_j^d\subset\R^{14}$ and collections of zonotope $\tilde\RR_{j^\text{h2l}}^d,\tilde\RR_{j^\text{l2h}}^d\subset P(\R^{14})$ as
%     \begin{align}
%         \tilde\RR_{j^\text{h2l}}^d:=\{\tilde\RR_{j^\text{h2l}}^{\text{hi},d}, \tilde\RR_{j_1^\text{h2l}}^{\text{lo},d},\tilde\RR_{j_1^\text{h2l}+1}^{\text{lo},d},\cdots,\tilde\RR_{j_2^\text{h2l}}^{\text{lo},d}\}\\
%         \tilde\RR_{j^\text{l2h}}^d:=\{\tilde\RR_{j^\text{l2h}}^{\text{lo},d}, \tilde\RR_{j_1^\text{l2h}}^{\text{hi},d},\tilde\RR_{j_1^\text{l2h}+1}^{\text{hi},d},\cdots,\tilde\RR_{j_2^\text{l2h}}^{\text{hi},d}\}
%     \end{align}
%     such that 
%     \begin{equation}
%         \Z_{xy}^d\subseteq \bigcup_{\tilde\RR\in\tilde\RR_T^d}\pi_{xyp}(\tilde\RR)
%     \end{equation}
%     where
%     \begin{equation}
%         \tilde \RR_T^d= \left(\bigcup_{j\in\J^d}\{\tilde\RR_j^d\}\right)\cup
%         \left(\bigcup_{j^\text{h2l}\in\J^{\text{h2l},d}}\tilde\RR_{j^\text{h2l}}^d\right)\cup
%         \left(\bigcup_{j^\text{l2h}\in\J^{\text{l2h},d}}\tilde\RR_{j^\text{l2h}}^d\right)
%     \end{equation}
%     as a collection of zonotopes.
    
%     % In $\R^{14}$ there exist zonotope $\tilde\RR_j$ for any $j\in\J$, zonotopes $\tilde\RR_{j^\text{h2l}}^\text{hi}, \tilde\RR_{j_1^\text{h2l}}^\text{lo},\tilde\RR_{j_1^\text{h2l}+1}^\text{lo},\cdots,\tilde\RR_{j_2^\text{h2l}}^\text{lo}$ for any $j^\text{h2l}=(j_1^\text{h2l},j_2^\text{h2l})\in\J^\text{h2l}$, and zonotopes $\tilde\RR_{j^\text{l2h}}^\text{lo}, \tilde\RR_{j_1^\text{l2h}}^\text{hi},\tilde\RR_{j_1^\text{l2h}+1}^\text{hi},\cdots,\tilde\RR_{j_2^\text{l2h}}^\text{hi}$ for any $j^\text{l2h}=(j_1^\text{l2h},j_2^\text{l2h})\in\J^\text{l2h}$
    
%     % % For any $j\in\J$, $j^\text{h2l}=(j_1^\text{h2l},j_2^\text{h2l})\in\J^\text{h2l}$ and $j^\text{l2h}=(j_1^\text{l2h},j_2^\text{l2h})\in\J^\text{l2h}$, there exist zonotopes $\tilde\RR_j,
%     % % \tilde\RR_{j^\text{h2l}}^\text{hi}, \tilde\RR_{j_1^\text{h2l}}^\text{lo},\tilde\RR_{j_1^\text{h2l}+1}^\text{lo},\cdots,\tilde\RR_{j_2^\text{h2l}}^\text{lo},
%     % % \tilde\RR_{j^\text{l2h}}^\text{lo}, \tilde\RR_{j_1^\text{l2h}}^\text{hi},\tilde\RR_{j_1^\text{l2h}+1}^\text{hi},\cdots,\tilde\RR_{j_2^\text{l2h}}^\text{hi}$ 

%     % There exist zonotope $\tilde\RR_j$ for all $j\in\J$, and set $\tilde\RR_{j^*}$ as a union of zonntopes for all $j^*\in\J^*$ such that $\Z_{xy}^d\subseteq \pi_{xyu}\left(\overline\Z_{xy}^d\right)$ where 
%     % % \begin{equation}
%     % %     \Z_{xy}^d\subseteq \pi_{xyu}\left(\overline\Z_{xy}^d\right)
%     % % \end{equation}
%     % % where
%     % \begin{equation}
%     % \overline\Z_{xy}^d:=\left(\bigcup_{j\in\J} \tilde\RR_j\right)\cup \left(\bigcup_{j^*\in\J^*} \tilde\RR_{j^*}\right).
%     % \end{equation}
% \end{thm}

% \jinsun{ATTENTION!!!!!!!!!!!!!!!!!!!!!! I've switched the next two subsections as I mentioned on slack}




\subsection{Slicing}

The FRS computed in the previous subsection contain the behavior of the hybrid vehicle dynamics model for all initial conditions belonging to $\Z_0$ and $\P$. 
To use this set during online optimization, \methodname{} plugs in the initial condition of the vehicle dynamics at time $\tz + \tplan$\jinsun{should it be just `time 0' since we've reset $\tz + \tplan$ as 0 always?} and then optimizes over the space of trajectory parameters. 
This subsection describes how to plug in the initial condition into the pre-computed FRS. 

Before describing how to plug in the initial condition into the FRS, we note the following useful property of the zonotopes $\RR_j$ that make up the FRS, which follows from Lemma 22 in \cite{holmes2020reachable}:
\begin{prop}
\label{prop: sliceable}
    Let $\{\RR_j = \zonocg{c_{\RR_j}}{G_{\RR_j}}\}_{j \in \J}$ be the set of zonotopes computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$.
    Then for any $j\in\J$, $G_{\RR_j}=[g_{\RR_j,1},g_{\RR_j,2},\ldots,g_{\RR_j,\ell_j}]$ has only one generator $g_{\RR,b_k}$ that has a nonzero element in the $k$-th dimension for each $k \in \{7, \ldots, (12 + n_p) \}$.
    In particular, $b_{k}\neq b_{k'}$ for $k \neq k'$. 
\end{prop}
\noindent We refer to the generators with a nonzero element in the $k$-th dimension for each $k \in \{7, \ldots, (12 + n_p) \}$ as a \emph{sliceable generator} of $\RR_j$ in the $k$-th dimension.
In other words, for each $\RR_j= \zonocg{c_{\RR_j}}{G_{\RR_j}}$, there are exactly $6 + n_p$ nonzero elements in the last  $6 + n_p$ rows of $G_{\RR_j}$, and none of these nonzero elements appear in the same row or column. 
By construction $\Zaug_0$ has exactly $6 + n_p$ generators, which are each sliceable.
Using Proposition \ref{prop: sliceable}, one can conclude that $\RR_j$ has no less than $6 + n_p$ generators (i.e., $\ell\geq 6 + n_p$). 

Proposition \ref{prop: sliceable} is powerful because it allows us to take a known $z_0 \in \Z_0$ and $p \in \P$ and plug them into the computed $\{\RR_j\}_{j\in\J}$ to generate a \emph{slice} of the conservative approximation of the FRS that includes the evolution of the hybrid vehicle dynamics model beginning from $z_0$ under trajectory parameter $p$.
In particular, one can plug the initial conditions into the sliceable generators as described in the following definition:
\begin{defn} \label{defn:slice}
Let $\{\RR_j = \zonocg{c_{\RR_j}}{G_{\RR_j}}\}_{j \in \J}$ be the set of zonotopes computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$\Review{.
Let}{ where} $G_{\RR_j}=[g_{\RR_j,1},g_{\RR_j,2},\ldots,\deleted{g_{\RR_j,\ell,}} \Review{}{ g_{\RR_j,{\ell_j}}}]$. \jinsun{Number of generators varies among $\RR_j$s.}
Without loss of generality, assume that the sliceable generators of each $\RR_j$ are the first $6+n_p$ columns of $G_{\RR_j}$.
In addition, without loss of generality assume that the sliceable generators are ordered so that the dimension in which the non-zero element appears is increasing. 
The \emph{slicing operator} $\slice: P(\R^{12 + n_p})\times\Z_0\times\P\rightarrow  P(\R^{12 + n_p})$ is defined as
\begin{equation}
\label{eq: slice def}
   \hspace*{-0.25cm} \slice( \RR_j,z_0,p) = \zonocg{c^\text{slc}}{[g_{\RR_j,(6 +n_p + 1)},\ldots,\deleted{g_{\RR_j,\ell,}} \Review{}{ g_{\RR_j,{\ell_j}}}]}
\end{equation}
where 
\begin{equation}
\label{eq: slice center}
\begin{split}
    c^\text{slc} = c_{\RR_j} + \sum_{k=7}^{12}&\frac{[z_0]_{(k-6)}-[c_{\RR_j}]_k}{[g_{\RR_j,(k-6)}]_k}g_{\RR_j,(k-6)} + \\ &+\sum_{k=13}^{12+n_p}\frac{[p]_{(k-12)}-[c_{\RR_j}]_k}{[g_{\RR_j,(k-6)}]_k}g_{\RR_j,(k-6)}.
\end{split}
\end{equation}
\end{defn}
\noindent Note, that in the interest of avoiding introducing novel notation, we have abused notation and assumed that the domain of $\slice$ is $P(\R^{12 + n_p})$ rather than the space of zonotopes in $P(\R^{12 + n_p})$. 
However, throuhgout this paper we only plug in zonotopes belonging to $P(\R^{12 + n_p})$ into the first argument of $\slice$.
% Proposition \ref{prop: sliceable} is attractive because the coefficients of sliceable generators are exact as long as $z_0$ and $p$ are known.
% To see this, without loss of generality assume $b_k=k-6$ for all $k\in\{7,8,\cdots,14\}$ and for all $\RR_j(d)=<c_{\RR},G_\RR>\in\RR_\J(d)$.
% That means the first 8 generators of $\RR_j(d)$ are the sliceable generators on the last 8 dimensions.
% Then by definition of zonotope, any point $z\in \RR_j(d)$ satisfies 
% \begin{equation}
% \label{eq: in zono}
%     [z]_k = [c_{\RR}]_i + \beta_{k-6}[g_{\RR}^{(k-6)}]_k, ~\forall k\in\{7,8,\cdots,14\}
% \end{equation}
% for some $\beta_{k-6}\in[-1,1]$.
% Thus if $z$ is given, $\beta_{k-6}$ for any $k\in\{7,8,\cdots,14\}$ can be specified as 
% \begin{equation}
% \label{eq: get coef}
%     \beta_{k-6} = \frac{[z]_k - [c_{\RR}]_i}{[g_{\RR}^{(k-6)}]_k}.
% \end{equation}


% Equality \eqref{eq: get coef} derived from Proposition \ref{prop: sliceable} allows us to generate a tighter prediction of ego vehicle's behavior with known initial condition $z_0$ and control parameter $p$ compared to $\cup_{j\in \J}\pi_{xy}( \RR_j(d))$.
% Define the \emph{slicing operator} $\slice:P(\R^{14})\times\Z_0\times\P\rightarrow P(\R^{14})$ as
% \begin{equation}
%     \slice( \RR_j(d),z_0,p) = \zonocg{c^\text{slc}}{[g_{\RR}^{(9)},g_{\RR}^{(10)},\cdots,g_{\RR}^{(\ell)}]}
% \end{equation}
% where 
% \begin{align}
% \label{eq: slice center}
%     c^\text{slc} = c_{\RR} + \sum_{k=7}^{12}&\frac{[z_0]_{k-6}-[c_{\RR}]_k}{[g_{\RR}^{(k-6)}]_k}g_{\RR}^{(k-6)} + \nonumber\\ &+\sum_{k=13}^{14}\frac{[p]_{k-12}-[c_{\RR}]_k}{[g_{\RR}^{(k-6)}]_k}g_{\RR}^{(k-6)}.
% \end{align}
Using this definition, one can prove the following useful property:
\begin{thm}
\label{thm: slice_is_good}
Let $\{\RR_j \}_{j \in \J}$ be the set of zonotopes computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$ and satisfy the statement of Definition \ref{defn:slice}.
    Then for any $j\in\J$, $z_0\in\Z_0$, and $p\in\P$,  $\slice( \RR_j,z_0,p)\subset \RR_j$.
    In addition, suppose $\zaug$ is a solution to $HS$ with initial condition $z_0$ and control parameter $p$.
    Then for each $j \in \J$ and $t \in T_j$
    \begin{equation}
        \zaug(t)\in \slice( \RR_j,z_0,p ).
    \end{equation}
\end{thm}
\begin{proof}
    \Review{}{Because $z_0$ and $p$ have zero dynamics in hybrid model $HS$, the area described by the last $6+n_p$ dimensions in $\RR_j$ for all $j\in \J$ is identical to $\Z_0\times\P$. 
    As a direct result of Proposition \ref{prop: sliceable} and assumptions in Definition \ref{defn:slice}, $\Z_0\times\P = \zonocg{c_j'}{G_j'}$ where $c_j' = \big[[c_{\RR_j}]_7, [c_{\RR_j}]_8, \cdots, [c_{\RR_j}]_{(12+n_p)}\big]^\top$ and $G_j' = \diag\left(\big[[g_{\RR_{j,1}}]_7, [g_{\RR_{j,2}}]_8, \cdots, [g_{\RR_{j,(6+n_p)}}]_{(12+n_p)}   \big]\right)$ for all $j\in\J$.
    Since $z_0\in \Z_0$ and $p\in\P$, by Definition \ref{def: zonotope} $\frac{[z_0]_{(k-6)}-[c_{\RR_j}]_k}{[g_{\RR_j,(k-6)}]_k} \in [-1,1]$ for all $k\in\{7,8,\cdots,12\}$, and $\frac{[p]_{(k-12)}-[c_{\RR_j}]_k}{[g_{\RR_j,(k-6)}]_k}\in[-1,1]$ for all $k\in\{13,14,\cdots,(12+n_p)\}$.}
    Notice $\slice( \RR_,z_0,p)$ is generated by specifying the coefficients of the first $6 + n_p$ generators in $\RR_j$ via \eqref{eq: slice center}, thus $\slice( \RR_j,z_0,p)\subset \RR_j$. \Review{by Definition \ref{def: zonotope}}{} \Ram{I'm missing something: why is it clear that the that coefficients will actually correspond to values between $[-1,1]$. Don't you need to prove that?}\jinsun{addressed}
    
    If a solution of $HS$ is initialized with initial condition $z_0$ and control parameter $p$, then vector that consists of the last $6+n_p$ dimensions in $\zaug$ remain fixed at $\begin{bmatrix} z_0 \\ p \end{bmatrix}$ for all $t\in T_j$ because of \eqref{eq: dyn tilde_z}.
    Notice $\RR_j$ is generated from CORA, so $\zaug(t)\in \RR_j$ for all $t \in T_j$ \Review{}{by Theorem \ref{thm: FRS over-approximation}.} \Ram{you need to cite a result that CORA generates conservative reachable sets for hybrid systems}\jinsun{addressed}
    \Review{then $\zaug(t)\in \cup_{j\in \J}\slice( \RR_j,z_0,p )$ for all $t \in [0,\tf]$ based on}{ Therefore by definition of the slicing operator in \eqref{eq: slice def}, $\zaug(t)\in \slice( \RR_j,z_0,p )$ for all $t \in T_j$.} \Ram{I am not sure why this last part is true. Seems like this needs to be rewritten}\jinsun{addressed}
\end{proof}





\subsection{Accounting for the Vehicle Footprint in the FRS}

The conservative representation of the FRS generated by CORA only accounts for the ego vehicle's center of mass because $HS$ treats the ego vehicle as a point mass.
To ensure not-at-fault behavior while planning using \methodname{}, one must account for the footprint of the ego vehicle, $\Oego$, as in Definition \ref{def: footprint}.

To do this, \Review{define the projection operator $\pi_h:\R^{12 + n_p}\rightarrow\R$, which projects a point in the augmented state space to the coordinate corresponding to the vehicle's heading (i.e. the third coordinate).
Note, that in the following discussion, we abuse notation and allow $\pi_h$ to be applied to subsets of $\R^{12+n_p}$. 
In that instance the function should be treated as being applied point-wise to elements of the set. 
Suppose that $\RR_j$ is generated by applying CORA as described in Section \ref{subsec: FRS computation}, then $\pi_h(\RR_j)$ gives a conservative representation to the ego-vehicle's heading state during the time interval $T_j$.
Notice in particular that $\pi_h(\RR_j)$ is a 1-dimensional zonotope that is equivalent to a 1-dimensional box of the form $[\hmid-\hrad, \hmid+\hrad]\subset\R$ with center $\hmid$ and radius $\hrad$}
{ define a projection operator $\pi_h: \{R_j\}_{j\in\J}\rightarrow P(\R)$ as $\pi_h(R_j) \mapsto \zonocg{[c_{R_j}]_3}{[G_{R_j}]_{3:}}$ where $R_j=\zonocg{c_{R_j}}{G_{R_j}}$ is some zonotope computed by CORA as described in Section \ref{subsec: FRS computation}.}
\jinsun{$[G_{R_j}]_{i:}$ is the $i$-th row of $G_{R_j}$, and this notation is introduced in preliminaries.}
% We have again abused notation and assume the domain of $\pi_h$ is $P(\R^{12+n_p})$ rather than the space of zonotopes in $P(\R^{12+n_p})$. 
% However in this paper $\pi_h$ is only operated on zonotopes in $P(\R^{12+n_p})$.
\Review{}{Suppose $\zaug$ is a solution to the hybrid system $HS$ starting from $\Zaug_0$ and $h(t)$ for all time indicates the trajectory of the 3rd dimension in $\zaug$.
Then by definition $\pi_h(\RR_j)$ is a zonotope and it conservatively approximates of the ego vehicle's heading during $T_j$.
Moreover, because $\pi_h(\RR_j)$ is a 1-dimensional zonotope, it can be rewritten as a 1-dimensional box $\Int(\hmid-\hrad, \hmid+\hrad)$ where $\hmid = [c_{\RR_j}]_3$ and $\hrad = \Sum(|[G_{\RR_j}]_{3:}|)$.} 
\Ram{why is $\pi_h(\RR_j)$ a zonotope? It feels like $\pi_h$ for a point and $\pi_h$ for a zonotope are actually very different functions, so I think we need a much more consequential definition.}\jinsun{addressed, btw the $\Sum$ operator and the absolute value operator $|\cdot|$ is introduced in preliminaries.}
We can then use $\pi_h$ to define a map to account for vehicle footprint within the FRS:
\begin{defn} \label{defn:footprint}
Let \Review{$\{\RR_j \}_{j \in \J}$ be the set of zonotopes}{ $\RR_j$ be the zonotope} computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$ \Review{}{for arbitrary $j\in\J$, and denote $\pi_h(\RR_j)$ as $\Int(\hmid-\hrad, \hmid+\hrad)$.}
Let $\SS \subset \W$ be a 2-dimensional box centered at the origin with length $\sqrt{L^2+W^2}$ and width $\frac{1}{2}L|\sin(\hrad)|+\frac{1}{2}W|\cos(\hrad)|$.
Define the \emph{rotation map} \Review{$\rot:P(\W)\times P(\R)\rightarrow P(\W)$}{ $\rot:P(\R)\rightarrow P(\W)$} as
\begin{equation}
\label{eq: def rot}
    \rot\big(\deleted{\Oego,}\pi_h(\RR_j)\big) = \begin{bmatrix}
        \cos(\hmid)& -\sin(\hmid)\\\sin(\hmid) & \cos(\hmid)
    \end{bmatrix} \SS.
\end{equation}
\jinsun{I delete $\Oego$ as an argument to $\rot$ because $\Oego$ is a constant and is only used implicitly in this definition.}
\end{defn}
\noindent Note that in the interest of simplicity, we have abused notation and assumed that the \Review{second}{} argument to $\rot$ is any subset of $\R$.
In fact, it must always be a $1$-dimensional box. 
In addition note that $\rot\big(\deleted{\Oego,}\pi_h(\RR_j)\big)$ is a zonotope because \Review{ $\SS$ can be written as a zonotope and $\hmid$ is constant}{ the 2-dimenional box $\SS$ is equivalent to a 2-dimensional zonotope and is multiplied by a matrix via \eqref{eq: zono-matrix mult}.} \Ram{this seems to be missing a proof or a citation}\jinsun{explained} 
\Ram{this picture is unacceptable.} \jinsun{need to ask why}
As shown in Fig. \ref{fig: ego rotate}, \Review{$\rot\big(\deleted{\Oego,}\pi_h(\RR_j)\big)$ outer approximates the area over which $\Oego$ sweeps according to $\pi_h(\RR_j)$.}{ $\rot\big(\pi_h(\RR_j)\big)$ has a heading equivalent to the mean value of $\pi_h(\RR_j)$. 
Moreover one can easily check by geometry that the area over which $\Oego$ sweeps according to $\pi_h(\RR_j)$ can be bounded by a box $\rot(\pi_h(\RR_j)$ with length $\sqrt{L^2+W^2}$ and width $\frac{1}{2}L|\sin(\hrad)|+\frac{1}{2}W|\cos(\hrad)|$ as defined in Definition \ref{defn:footprint}.}

\Review{}{Denote zonotope $\rot(\pi_h(\RR_j))$ as $\zonocg{c_\rot}{G_\rot}$.
Notice $\rot(\pi_h(\RR_j))$ in \eqref{eq: def rot} is a set in $\W$ rather than a higher dimensional space where $\RR_j$ exists, we then extend $\rot(\pi_h(\RR_j))$ to $\R^{12+n_p}$ as}
\begin{equation}
    \Review{}{\ROT(\pi_h(\RR_j)) := \left< \begin{bmatrix} c_\rot \\ 0_{(10+n_p)\times 1}\end{bmatrix},~
    \begin{bmatrix} G_\rot \\ 0_{(10+n_p)\times 2}\end{bmatrix}\right>.}
\end{equation}
\Review{}{In addition the following lemma holds.}
\begin{lem}
\label{lem: slice and rot}
    \Review{}{Let $\RR_j$ be the zonotope computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$ for arbitrary $j\in\J$, then for any $z_0\in\Z_0$ and $p\in\P$,}
    \begin{equation}
    \label{eq: slice and rot}
        \begin{split}
            \Review{}{\slice\big(\RR_j\oplus} & \Review{}{\ROT(\pi_h(\RR_j)), z_0, p\big) =} \\
            & \Review{}{= \slice(\RR_j, z_0, p)\oplus \ROT(\pi_h(\RR_j)).}
        \end{split}    
    \end{equation}
\end{lem}
\begin{proof}
    \Review{}{Because $\ROT(\pi_h(\RR_j))$ is a constant with respect to $z_0$ and $p$ by definition, $\RR_j$ shares the same sliceable generators as $\RR_j\oplus\ROT(\pi_h(\RR_j))$.
    Notice the slice operator only affect sliceable generators and keep all the rest generators, thus \eqref{eq: slice and rot} holds.}
\end{proof}




% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.49\columnwidth}
%          \centering
%          \includegraphics[trim={0.5cm, 1.5cm, 20.5cm, 7cm},clip,width=\textwidth]{figures/rotate_ego.pdf}
%          \caption{}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\columnwidth}
%          \centering
%          \includegraphics[trim={15.2cm, 1.5cm, 6cm, 7cm},clip,width=\textwidth]{figures/rotate_ego.pdf}
%          \caption{}
%      \end{subfigure}
%     \caption{Rotation of ego vehicle's footprint. 
%     In (a), the ego vehicle together with its footprint rotate within range $\pi_h(\RR_j)$.
%     The ego vehicle with heading equals to the mean value of $\pi_h(\RR_j)$ is bounded by the box with solid black boundaries.
%     Maximum and minimum rotated headings are marked by gray straight lines, and the area the ego vehicle's footprint sweeps is colored in gray.
%     In (b), the gray area that the ego vehicle's footprint sweeps while it rotates within the heading range $\pi_h(\RR_j)$ is bounded by box $\rot\big(\pi_h(\RR_j)\big)$ with dashed black boundaries. 
%     Note $\rot\big(\pi_h(\RR_j)\big)$ has a heading equivalent to the mean value of $\pi_h(\RR_j)$.}
%     \label{fig: ego rotate}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[trim=0cm 1cm 18cm 6.5cm, clip,width=0.8\columnwidth,clip=true]{figures/rotate_ego_v2.pdf}
    \caption{Rotation of the ego vehicle and its footprint within range $\pi_h(\RR_j)$. The ego vehicle with heading equals to the mean value of $\pi_h(\RR_j)$ is bounded by the box with solid black boundaries.
    Maximum and minimum rotated headings are marked by gray straight lines.
    The area the ego vehicle's footprint sweeps is colored in grey, and is bounded by box $\rot\big(\pi_h(\RR_j)\big)$ with dashed black boundaries.}
    \label{fig: ego rotate}
\end{figure}







\Review{}{We abuse the notation and allow the projection operator $\pi_{xy}$ to be applied to zonotopes in $P(\R^{12+n_p})$.}
The definition of \Review{$\rot$}{ $\ROT(\pi_h(\RR_j))$} can be used to extend the FRS to account for the vehicle footprint as proven in the following lemma:
\begin{lem} \label{lem:footprint}
Let $\{\RR_j\}_{j \in \J}$ be the set of zonotopes computed by CORA under the hybrid vehicle dynamics model beginning from $\Zaug_0$.
Let $\zaug$ be a solution to $HS$ with initial condition $z_0$ and control parameter $p$ and 
let $\xi:P(\R^{12 + n_p})\times \Z_0\times\P\rightarrow P(\W)$ be defined as
\begin{equation}
\begin{split}
    \deleted{\xi(\RR_j,z_0,p) = \pi_{xy}\big(\slice(\RR_j,z_0,p)\big)\oplus}\\
    \deleted{ \oplus \rot\big(\Oego, \pi_h(\slice(\RR_j,z_0,p)\big).}
    \end{split}
\end{equation}
\begin{equation}
\label{eq: xi def}
    \Review{}{\xi(\RR_j,z_0,p) = \pi_{xy}\Big(\slice\big(\RR_j\oplus\ROT(\pi_h(\RR_j)), z_0, p\big)\Big).}
\end{equation}
Then $\xi(\RR_j,z_0,p)$ is a zonotope and for all $j \in \J$ and $t \in T_j$, the vehicle footprint oriented appropriately and centered at $\zaug(t)$ is contained within $\xi(\RR_j,z_0,p)$.
\end{lem}
\begin{proof}
\Ram{need this to be proven.}\jinsun{addressed}
\Review{}{By definition $\slice(\RR_j, z_0, p)$ and $\ROT(\pi_h(\RR_j))$ are both zonotopes, thus $\slice\big(\RR_j\oplus\ROT(\pi_h(\RR_j)), z_0, p\big)$ is a zonotope per \eqref{eq: slice and rot}.
For simplicity denote $\slice\big(\RR_j\oplus\ROT(\pi_h(\RR_j)), z_0, p\big)$ as $\zonocg{c''}{G''}$, then $\xi(\RR_j,z_0,p)$ is a zonotope because}
\begin{equation}
    \Review{}{\pi_{xy}\big(\zonocg{c''}{G''}\big) = \left< \begin{bmatrix} [c'']_1 \\ [c'']_2 \end{bmatrix},~ \begin{bmatrix}[G'']_{1:} \\ [G'']_{2:}\end{bmatrix} \right>.}
\end{equation}


\Review{}{Note $\pi_{xy}\big(\ROT(\pi_h(\RR_j))\big)=\rot(\pi_h(\RR_j))$, and by definition of $\pi_{xy}$ it can be easily checked that $\pi_{xy}(\mathcal A_1\oplus\mathcal A_2) = \pi_{xy}(\mathcal A_1)\oplus\pi_{xy}(\mathcal A_2)$ for any zonotopes $\mathcal A_1, \mathcal A_2\subset \R^{12+n_p}$.
Then by Lemma \ref{lem: slice and rot},}
\begin{equation}
\label{eq: xi = pi_slice + rot}
    \Review{}{\xi(\RR_j,z_0,p) = \pi_{xy}\big(\slice(\RR_j, z_0, p)\big)\oplus\rot(\pi_h(\RR_j)).}
\end{equation}

\Review{}{By Theorem \ref{thm: slice_is_good} for any $t\in T_j$ and $j\in\J$,  $\zaug(t)\in\slice(\RR_j,z_0,p)\subset\RR_j$, then $h(t)\in\pi_h(\RR_j)$.
Because $\rot(\pi_h(\RR_j))$ by construction outer approximates the area over which $\Oego$ sweeps according to all possible heading of the ego vehicle during $T_j$,  then $\xi(\RR_j,z_0,p)$ contains the vehicle footprint oriented according to $\pi_h(\RR_j)$ and centered at $\pi_{xy}(\zaug(t))$ during $T_j$.
}
\end{proof}
Again note that in the interest of simplicity we have abused notation and assumed that the first argument to $\xi$ is any subset of $\R^{12+n_p}$.
However, this argument is always a zonotope in  $\R^{12+n_p}$.

\begin{rem}
\Review{}{Other than $\xi(\RR_j,z_0,p)$ one can have a tighter embedding of the vehicle footprint in the FRS as}
\begin{equation}
    \begin{split}
        \Review{}{\xi'(\RR_j,z_0,p):=\pi_{xy}\big(\slice(\RR_j, z_0, p)\big)\oplus}\\
        \Review{}{\oplus \rot\big(\pi_h(\slice(\RR_j, z_0, p))\big).}
    \end{split}
\end{equation}
\Review{}{In other words, instead of rotating the vehicle footprint according to all possible heading in $\pi_h(\RR_j)$ as $\xi(\RR_j,z_0,p)$ does, $\xi'(\RR_j,z_0,p)$ only rotates the vehicle footprint according to vehicle's heading with respect to particular $z_0$ and $p$.
However the rotational piece in $\xi'(\RR_j,z_0,p)$ requires values of $z_0$ and $p$ that are only available online, while $\xi(\RR_j,z_0,p)$ as in \eqref{eq: xi def} allows us to compute $\ROT(\pi_h(\RR_j))$ completely offline.
Thus for computational efficiency in real-time, we use $\xi(\RR_j,z_0,p)$ to account for the ego vehicle's footprint. 
Furthermore, $\xi$ results in nearly linear constraints on obstacle avoidance as shown in Section \ref{subsec: constraint}.}
\end{rem}








